Beep: Fine-grained Fix Localization by Learning to Predict Buggy Code Elements

Software Fault Localization refers to the activity of finding code elements (e.g., statements) that are related to a software failure. The state-of-the-art fault localization techniques, however, produce coarse-grained results that can deter manual debugging or mislead automated repair tools. In this work, we focus specifically on the fine-grained identification of code elements (i.e., tokens) that must be changed to fix a buggy program: we refer to it as fix localization. This paper introduces a neural network architecture (named Beep) that builds on AST paths to predict the buggy code element as well as the change action that must be applied to repair a program. Leveraging massive data of bugs and patches within the CoCoNut dataset, we trained a model that was (1) effective in localizing the buggy tokens with the Mean First Rank significantly higher than a statistics based baseline and a machine learning-based baseline, and (2) effective in predicting the repair operators (with the associated buggy code elements) with a Recall@1= 30-45% and the Mean First Rank=7-12 (evaluated by CoCoNut, ManySStuBs4J, and Defects4J datasets). To showcase how fine-grained fix localization can help program repair, we employ it in two repair pipelines where we use either a code completion engine to predict the correct token or a set of heuristics to search for the suitable donor code. A key strength of accurate fix localization for program repair is that it reduces the chance of patch overfitting, a challenge in generate-and-validate automated program repair: both two repair pipelines achieve a correctness ratio of 100%, i.e., all generated patches are found to be correct. Moreover, accurate fix localization helps enhance the efficiency of program repair.

==> tables/RQ1-result.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Prediction Results when Only Considering Elements}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{c|cccc}
    \toprule
    Dataset & Top-1 & Top-3 & Top-5 & MFR \\
    \midrule
    CoCoNut  & 46.94\% & 74.24\% & 85.49\% & 95.20\% & 3.87 \\
    ManySStuBs4J   & 30.72\% & 56.41\% & 72.60\% & 90.10\% & 6.69 \\
    \bottomrule
    \end{tabular}%
    }
    \label{table:RQ1-result}
\end{table}%


==> tables/RQ4-result.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htp]
  \centering
  \caption{Comparison of Model Designs.}
  \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{c|r|ccccc|ccccc}
    \toprule
    \multirow{2}{*}{\bf Prediction objective} & \multicolumn{1}{c|}{\multirow{2}{*}{\bf Model Design}} & \multicolumn{5}{c|}{\bf CoCoNut}          & \multicolumn{5}{c}{\bf ManySStuBs4J} \\
\cline{3-12}          &       & Top-1 & Top-5 & Top-10 & Top-20 & MFR   & Top-1 & Top-5 & Top-10 & Top-20 & MFR \\
    \hline
    \multirow{4}[1]{*}{Buggy code element} & no token splitting & 44.5\% & 72.0\% & 83.1\% & 92.6\% & 4.7  & 28.6\% & 53.1\% & 53.1\% & 87.7\% & 7.2 \\
          & no AST nodes & 46.5\% & 74.0\% & 85.3\% & {\bf95.4\%} & {\bf3.9}  & 29.5\% & 49.3\% & 68.7\% & 86.5\% & 7.2 \\
          & no fully-connected layer & {\bf47.7}\% & {\bf74.7}\% & 85.3\% & 94.7\% & 4.0  & 29.1\% & 45.2\% & 55.7\% & 71.9\% & 7.0 \\
          & BEP   & 46.9\% & 74.2\% & {\bf85.5\%} & 95.2\% & {\bf3.9}  & {\bf30.7\%} & {\bf56.4\%} & {\bf72.6\%} & {\bf90.1\%} & {\bf6.7} \\\hline
    \multirow{4}[1]{*}{Element + Operator} & no token splitting & 41.8\% & 63.3\% & 71.3\% & 79.4\% & 13.5 & 26.8\% & 45.5\% & 58.7\% & 74.7\% & 16.4 \\
          & no AST nodes & 43.8\% & 67.1\% & 77.0\% & 86.9\% & 7.6  & 27.7\% & 48.5\% & 62.2\% & 77.3\% & 12.3 \\
          & no fully-connected layer & {\bf44.8\%} & {\bf68.0\%} & 77.2\% & 86.1\% & 8.3  & 27.8\% & 40.8\% & 48.8\% & 62.0\% & 12.6 \\
          & BEP   & 44.6\% & 67.8\% & {\bf77.9\%} & {\bf87.6\%} & {\bf7.5}  & {\bf29.7\%} & {\bf50.8\%} & {\bf63.7\%} & {\bf79.3\%} & {\bf11.5} \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:rq4-result}%
\end{table*}%


==> tables/extra-single-token-bug.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Proportion of single-token bugs in large-scale defect benchmarks.}
  \resizebox{1\linewidth}{!}{
  \begin{threeparttable}
    \begin{tabular}{L{30mm}|R{20mm}R{35mm}}
    \toprule
    \textbf{Datasets} & \textbf{\# all bugs} & \textbf{\# Single-token bugs}  \\
    \hline
    CoCoNut$^\dagger$  & 436,676 & 179,037 ($\approx 41\%$) \\
    ManySStuBs4J$^\dagger$   & 26,406  &  6,787 ($\approx 26\%$) \\
    \bottomrule
    \end{tabular}%
    {
    $^\dagger$Statistics of both datasets are calculated after our preprocessing. For CoCoNut, we removed all the empty lines and duplicate ones. For ManySStuBs4J, we disregarded instances from test code.
    }
    \end{threeparttable}
    }
    \label{tab:extra-single-token}
    \vspace{-1mm}
\end{table}%



==> tables/multiple-token-bugs-performance.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table}[htbp]
%  \vspace{0.3cm}
%  \centering
%  \caption{Prediction Results of \toolname on 20 Multiple Token Bugs in Defects4J.}
%   \resizebox{1\linewidth}{!}
%  {
%  \begin{threeparttable}
%    \begin{tabular}{cccc}
%    \toprule
%    \textbf{Top-1} & \textbf{Top-5} & \textbf{Top-10} & \textbf{Top-20}  \\
%    \hline
%    6 & 13 & 18 & 20 \\
%    \bottomrule
%    \end{tabular}%
%    {
%    }
%    \end{threeparttable}
%    }
%    \label{tab:multiple-token-bugs}
%\vspace{0.1cm}
%\end{table}%

==> tables/repair_result.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\iffalse
\begin{table}[htbp]
  \centering
  \caption{Comparison with State-of-the-art APR Approaches.}
  \resizebox{1\linewidth}{!}{
  \begin{threeparttable}
    \begin{tabular}{lcccc}
    \toprule
    Tool  & \multicolumn{1}{p{6.375em}}{Defects4J-V2.0\newline{}835 bugs} & \multicolumn{1}{p{4.19em}}{Bears\newline{}251 bugs} & \multicolumn{1}{p{4.19em}}{QuixBugs\newline{}40 bugs} & \multicolumn{1}{p{4.19em}}{CR(\%)} \\
    \midrule
    LSRepair~\cite{liu2018lsrepair} & 19/37 & -     & -     & 51.4 \\
    DLFix~\cite{li2020dlfix} & 29/65 & -     & -     & 44.6 \\
    JAID~\cite{chen2017contract}  & 9/31  & -     & -     & 29 \\
    HDRepair~\cite{le2016history} & 13/23 & -     & -     & 56.5 \\
    SketchFix~\cite{hua2018towards} & 19/26 & -     & -     & 73.1 \\
    ssFix~\cite{xin2017leveraging} & 20/60 & -     & -     & 33.3 \\
    CapGen~\cite{wen2018context} & 21/25 & -     & -     & \textbf{84} \\
    ConFix~\cite{kim2019automatic} & 22/92 & -     & -     & 23.9 \\
    Elixir~\cite{saha2017elixir} & 26/41 & -     & -     & 63.4 \\
    Hercules~\cite{saha2019harnessing} & 49/72 & -     & -     & 68.1 \\
    Nopol~\cite{xuan2017nopol} & 2/9   & ?/1   & 1/4   & 23.1 \\
    DynaMoth~\cite{durieux2016dynamoth} & 3/13  & 0/0   & ?/2   & 23.1 \\
    jKali~\cite{martinez2016astor} & 2/8   & ?/10  & 1/2   & 30 \\
    Kali-A~\cite{yuan2018arja} & 6/42 & ?/15 & ?/2 & 14.3 \\
    jGenProg~\cite{martinez2016astor} & 6/16  & ?/13  & 0/2   & 33.3 \\
    GenProg-A~\cite{yuan2018arja} & 7/29 & ?/1 & ?/4 & 24.1 \\
    jMutRepair~\cite{martinez2016astor} & 5/11  & ?/7   & ?/3   & 45.5 \\
    Cardumen~\cite{martinez2018ultra} & 2/16  & ?/13  & ?/4   & 12.5 \\
    RSRepair-A~\cite{yuan2018arja} & 10/24 & ?/1   & 2/4   & 42.9 \\
    ARJA~\cite{yuan2018arja}  & 12/36 & ?/12  & ?/4   & 33.3 \\
    SequenceR~\cite{chen2019sequencer} & 12/19 & -     & -     & 63.2 \\
    ACS~\cite{xiong2017precise}   & 16/21 & -     & -     & 76.2 \\
    SimFix~\cite{jiang2018shaping} & 27/50 & -     & -     & 54 \\
    kPAR~\cite{liu2019you}  & 29/56 & -     & -     & 51.8 \\
    AVATAR~\cite{liu2019avatar} & 29/50 & -     & -     & 58 \\
    FixMiner~\cite{koyuncu2020fixminer} & 34/62 & -     & -     & 54.8 \\
    TBar~\cite{liu2019tbar}  & 52/85 & -     & -     & 61.2 \\
    CoCoNut~\cite{lutellier2020coconut} & 44/85 & -     & 13/20 & 54.3 \\
    \midrule
    Our Method (not fixed by others) & 19/19 (3) & 2/2 (2) & 4/4 (0) & \textbf{100} \\
    \bottomrule
    \end{tabular}%
    {
    Data of other tools are directly extracted from previous studies \cite{liu2020efficiency,lutellier2020coconut,durieux2019empirical}. x/y represents the tool generates y plausible patches among which x are correct on this benchmark.
    ``?'' means in the study \cite{durieux2019empirical}, authors do not pay attention to patch correctness and thus these data are unavailable. ``-'' means no relevant information. We discard Closure-63 and Closure-93 since they are listed as duplicated ones on the official webpage of Defects4J-V2.0\footnote{\url{https://github.com/rjust/defects4j/tree/master}}.
    }
    \end{threeparttable}
    }
  \label{tab:repair-result}%
\end{table}%
\fi


\begin{table}[htbp]
  \centering
  \caption{Comparison with state-of-the-art APR tools on fixing single-token real-world bugs.}
  \resizebox{1\linewidth}{!}{
  \begin{threeparttable}
    \begin{tabular}{lccccr}
    \toprule
    {\bf APR Tool} & {\bf Defects4J} & {\bf Bears} & {\bf QuixBugs} & {\bf Bugs.jar} & {\bf CR(\%)} \\
    \midrule
    LSRepair~\cite{liu2018lsrepair} & 4/7   & -     & - &-    & 57.1 \\
    JAID~\cite{chen2017contract}  & 8/8   & -     & - &-    & \textbf{100} \\
    SketchFix~\cite{hua2018towards} & 13/15 & -     & -  &-    & 86.7 \\
    ssFix~\cite{xin2017leveraging} & 11/12 & -     & -  &-   & 91.7 \\
    CapGen~\cite{wen2018context} & 15/17 & -     & - &-     & 88.2 \\
    ConFix~\cite{kim2019automatic} & 14/22 & -     & - &-    & 63.6 \\
    Elixir~\cite{saha2017elixir} & 13/14 & -     & - &-     & 92.9 \\
    NPEFix~\cite{durieux2017dynamic} & 0/2 & 0/0 & 0/1 & 0/0 & 0 \\
    DLFix~\cite{li2020dlfix} & 20/- & - & - & - & - \\
    HDRepair~\cite{xuan2016history} & 13/- & - & - & - & - \\
    PraPR$^\dagger$~\cite{ghanbari2019practical} & 23/26 & - & - & - & 88.5 \\
    GenPat~\cite{jiang2019inferring} & 6/9 & - & - & - & 66.7 \\
    \bottomrule
    Nopol~\cite{xuan2017nopol} & 0/2   & 0/0   & 0/1  & 0/0 & 0 \\
    DynaMoth~\cite{durieux2016dynamoth} & 1/2   & 0/0   & 1/1  &0/2  & 40 \\
    jKali~\cite{martinez2016astor} & 0/2   & 0/1   & 1/1  & 0/0 & 25 \\
    Kali-A~\cite{yuan2018arja} & 0/5   & 0/1   & 1/1 & 0/0  & 14.3 \\
    jGenProg~\cite{martinez2016astor} & 2/4   & 0/1   & 0/0 & 0/0  & 40 \\
    GenProg-A~\cite{yuan2018arja} & 2/5   & 0/0   & 0/0 & 0/0  & 40 \\
    jMutRepair~\cite{martinez2016astor} & 4/4   & 0/0   & 2/3 & 0/0  & 85.7 \\
    Cardumen~\cite{martinez2018ultra} & 2/6   & 0/1   & 0/0 & 0/0  & 28.6 \\
    RSRepair-A~\cite{yuan2018arja} & 3/8   & 0/0   & 1/1 & 0/0  & 44.4 \\
    ARJA~\cite{yuan2018arja}  & 3/7   & 0/1   & 1/1 & 0/0  & 44.4 \\
    SequenceR~\cite{chen2019sequencer} & 11/13 & -     & -  & -   & 84.6 \\
    ACS~\cite{xiong2017precise}   & 3/3   & -     & -  & -   & \textbf{100} \\
    SimFix~\cite{jiang2018shaping} & 10/14 & -     & -  & -   & 71.4 \\
    kPAR~\cite{liu2019you}  & 12/14 & -     & -  & -   & 85.7 \\
    AVATAR~\cite{liu2019avatar} & 12/13 & -     & -  & -   & 92.3 \\
    FixMiner~\cite{koyuncu2020fixminer} & 17/20 & -     & -  & -   & 85 \\
    TBar~\cite{liu2019tbar}  & 19/20 & -     & -  & -   & 95 \\
    CoCoNut~\cite{lutellier2020coconut} & 19/- & - & 8/- & - & - \\
    CURE~\cite{jiang2021cure} & 22/- & - & 9/- & - & - \\
    \midrule
    \toolname + Heuristic & 18/18 & 0/0 & 5/5 & 6/6 & 100 \\
    Ground-truth buggy line + \ACG & 1/1 & 0/0 & 0/0 & 1/1 & 100 \\
    \midrule
    \rowcolor{grey}\repairtoolname (\#bugs not fixed by others) & 19/19 (4) & 2/2 (2) & 4/4 (0) & 5/5 (4) & \textbf{100} \\
    \bottomrule
    \end{tabular}%
    {Data of other tools are extracted from the original papers or some recent empirical studies \cite{liu2020efficiency,durieux2019empirical}. x/y represents the tool generates y plausible patches among which x are correct on this benchmark.
     ``-'' means no relevant information (for DLFix, HDRepair, CoCoNut, and CURE, information is only available for correctly fixed bugs).
     The first 12 APR tools above the dividing line are configured with normal spectrum-based fault localization, while the remaining 19 APR tools are fed with perfect fault localization (i.e., buggy lines). We do not consider the two alternative approaches when calculating number of bugs that are exclusively fixed by \repairtoolname. $^\dagger$PraPR was evaluated on Defects4J-v2.0.
    }
    \end{threeparttable}
    }
  \label{tab:repair-result}%
\end{table}%




==> tables/single-token-bug-performance.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Proportion of single-token bugs in APR benchmarks and their fix rate by the state of the art$^\star$.}
    \resizebox{1\linewidth}{!}{
    \begin{threeparttable}
    \begin{tabular}{l|c|ccc}
    \toprule
    \multicolumn{2}{c|}{\bf Benchmark}   & \multicolumn{3}{c}{\textbf{Single-token bugs }}  \\
       \hline
 \multirow{2}{*}{\textbf{Name}} &  \multirow{2}{*}{\textbf{\# all bugs}}  & \textbf{\# Single-token}  & \textbf{\# plausibly} & \textbf{\# correctly} \\
 & & \textbf{bugs} & \textbf{fixed} & \textbf{fixed}\\
    \hline%midrule
    \multicolumn{1}{l|}{Defects4J-1.4~\cite{just2014defects4j}} &391$^\dagger$  & 39 ($\approx 10\%$)   & 31    & 31 \\
    \multicolumn{1}{l|}{Bears~\cite{madeiral2019bears}} &251 & 6 ($\approx 2\%$)     & 1     & 0 \\
    \multicolumn{1}{l|}{QuixBugs~\cite{lin2017quixbugs}} & 40 & 9 ($\approx 22\%$)    & 3     & 2 \\
    \multicolumn{1}{l|}{Bugs.jar~\cite{saha2018bugs}} & 1,011$^\ddagger$  & 31 ($\approx 3\%$)    & 2     & 0 \\
    %\multicolumn{1}{r|}{Defects4J-2.0$^\dagger$} &444 & 23    & -     & - \\
    \hline
    Total & 1,697  & 88  ($\approx 5\%$)   & 37    & 33 \\
    \bottomrule
    \end{tabular}%
    {%\footnotesize
    %$^\dagger$ This row only illustrates the newly-added bugs of Defects4J-V2.0 compared with the previous version. Data are all 0 since no tool has been evaluated on them. 
    $^\star$We aggregated data on 30 Java APR tools whose execution results are publicly reported by the authors or by other studies. See Table~\ref{tab:repair-result} for all details.
    \\
    $^\dagger$We discard in this study 4 duplicated bugs listed on the homepage of \protect Defects4J\protect\footnotemark.
    \\
    $^\ddagger$We also discard {\tt Math} project in Bugs.jar since it has been included in Defects4J.
    }
\end{threeparttable}
    }
  \label{tab:single-token-bug performance}%
  \vspace{-1mm}
\end{table}%
\footnotetext{\url{https://github.com/rjust/defects4j/tree/master}}

